Nonlinear Stochastic Optimal Control and Optimal Stopping using the Fokker-Planck Transformation

In this paper, we develop a theoretical framework for nonlinear stochastic optimal control problems with optimal stopping by establishing a density-based deterministic representation of the underlying diffusion. For state-independent diffusion, we rewrite the controlled Fokker-Planck equation as a continuity equation driven by a score-corrected velocity field, yielding a deterministic characteristic dynamics that reproduces the marginal law of the stochastic system. Leveraging Stein-type identities, we show that the associated distributional dynamic programming equation admits the same second-order differential operator as the distributional stochastic Hamilton-Jacobi-Bellman formulation. Building on this representation, we formulate an optimal control problem with state-dependent terminal-time assignment and terminal distributional constraints and derive the first-order necessary conditions using variational analysis. We present the conditions both for a common terminal time and for the general case of state-dependent stopping.

==> sections/Conclusion.tex <==
\section{Conclusion}


\blue{We have developed a density-based framework for nonlinear stochastic optimal control problems with optimal stopping and
terminal distributional constraints.
%
The central step rewrites the controlled Fokker–Planck
equation as a continuity equation whose velocity is the original drift minus one-half of the diffusion covariance multiplied by the score of the alive density. 
%
Integration by parts then converts
the score-dependent contributions into diffusion terms in the distributional equations, while the absorbing-boundary flux records when and where stopping occurs. 
%
This representation
provides the basis for the variational analysis of control and stopping under the stated regularity and characteristic-representation assumptions. Future work will focus on developing scalable,
sampling-based numerical methods for high-dimensional problems, including indirect physics-informed approaches that combine the optimality conditions with score-matching algorithms.}



\section*{Acknowledgement}

Partial support for this work has been provided by NSF award 2551281. The authors also acknowledge insightful feedback by Tryphon T Georgiou on an early version of this manuscript.
